Model-Driven Requirements for Humans-on-the-Loop Multi-UAV Missions

The use of semi-autonomous Unmanned Aerial Vehicles (UAVs or drones) to support emergency response scenarios, such as fire surveillance and search-and-rescue, has the potential for huge societal benefits. Onboard sensors and artificial intelligence (AI) allow these UAVs to operate autonomously in the environment. However, human intelligence and domain expertise are crucial in planning and guiding UAVs to accomplish the mission. Therefore, humans and multiple UAVs need to collaborate as a team to conduct a time-critical mission successfully. We propose a meta-model to describe interactions among the human operators and the autonomous swarm of UAVs. The meta-model also provides a language to describe the roles of UAVs and humans and the autonomous decisions. We complement the meta-model with a template of requirements elicitation questions to derive models for specific missions. We also identify common scenarios where humans should collaborate with UAVs to augment the autonomy of the UAVs. We introduce the meta-model and the requirements elicitation process with examples drawn from a search-and-rescue mission in which multiple UAVs collaborate with humans to respond to the emergency. We then apply it to a second scenario in which UAVs support first responders in fighting a structural fire. Our results show that the meta-model and the template of questions support the modeling of the human-on-the-loop human interactions for these complex missions, suggesting that it is a useful tool for modeling the human-on-the-loop interactions for multi-UAVs missions.

==> TODO.tex <==
Things we need to do once we have a final draft:

1. Check for consistency of UAV vs. Agent use.  We have agreed to use UAV in our examles, and Agent in general discussion.

2. Check for the first use/intro of acronyms.

3. Discuss interaction points vs. points of intervention.  JP suggested this; however, I (JCH) think that intervention points are a subset of interaction points.  Let's change it everywhere it makes sense i.e., not for information exchange, but for direct commands and for lowering/raising autonomy.

4. Discuss how direct commands are implemented. It isn't enough to just change a role.

5. Consistency in how we describe the models.  What do we call each level?   What is an M1 level actually called? In UML an Object Diagram seems to be instantiated, while our diagrams are more conceptual Object Diagrams? What are they called?


==> prototype.tex <==
\section{System Design}

In this section, we describe the design of collaboration actions for the goal-oriented agents following the Belief-Desire-Intent(BDI) model. BDI agents are one of the most popular models inspired by the theory of human practical reasoning. Different architectures exist to implement the BDI agents such as JACK \cite{howden2001jack}, JADEX \cite{pokahr2005jadex}, and AgentSpeak \cite{rao1996agentspeak}. JADEX provides an open-source java environment to simulate intelligent agents. We choose to implement the core execution model of JADEX in python so that we can interface the implementation easily with our existing system. The \textit{beliefs} of BDI agents represent their knowledge of the environment. Multiple agents communicates to exchange their beliefs with each other. \textit{Desires} represents the state of the agent that it wishes to achieve. The commitment to a particular desire represents the goal of an agent. Each goal includes plans  that an agent  adopts to pursue the goal. Intentions are the series of actions in a plan that an agent executes to achieve the goal successfully. Now we map these concepts to the human-on-the-loop collaboration actions discussed in section \ref{sec:Actions}. 
%  using  Spade \footnote{https://pypi.org/project/spade/} library


\textbf{Share knowledge}: Beliefs represents the knowledge-base of the BDI agents. Therefore, in our implementation, we categorize beliefs into three parts based on the level of their awareness about the environment. These levels corresponds to different levels of situational awareness. Level-1 belief variables represents the existence of objects in the environment such as location of fire-fighters and rescue boats, and assigned search area in a river search-and-rescue mission. Level-2 beliefs represent the context of the situation such as whether a victim is identified in the river. Finally level-3 beliefs variables include the probable estimates about the future state of the environment such as estimated arrival times of rescue-boats and flotation devices. All these beliefs variables construct the knowledge-base and situation awareness of the agent. In our implementation, human actions to share the knowledge of the environment results in updating the beliefs of agents at different levels. These updates in the belief state at run-time triggers the agent to adapt their behavior accordingly. 

\textbf{Feedback and Commands}: \textit{Plans} represents the behavioral aspect of the BDI agent. An agent might have multiple plans to achieve a single goal. Therefore, the agents uses its reasoning engine to select one of the applicable plans. A change in the goal of the agent trigger it to re-evaluate the plans and select one that is appropriate for achieving the new goal. In our system, we implement Feedback and Commands to influences the goal. A command to the BDI agent directly manipulates the  goal of the agent which results in adoption of new intents or actions. For example, a UAV currently searching an area, upon receiving a command to replace another UAV, causes it to abort the current goal and adopt a new goal. On the other hand, a feedback from human operator on the current execution of actions will cause an update in the parameters of goals and intents of the UAV. This update in the parameter in intended to improve the execution of a goal.

% \textbf{Consistent Awareness:} we use "query goals" provided by JAdex to generate the explanations for the current behavior of the UAV. 

\textbf{Autonomy Levels}: The dispatcher in the JADEX execution model is responsible to select an appropriate plan in response to an event. The selection of a plan for execution is done in two steps. First, the dispatcher generates a list of applicable plans by matching the pre-conditions of every plan against the event.  The meta-level reasoning in the next step select an appropriate plan for execution. In scenario S5, the applicable plans against the event \emph{low battery} while tracking the victims are either continue tracking the victim or launch the RTL for safety purpose. In such scenarios, the human action to lower the autonomy levels in our implementation dynamically modifies the applicability of a plan for an event. This restricts the dispatcher from selecting the RTL as an applicable plan while tracking the victim. The human operator can dynamically modify the applicability of plans to apply constraints on the mission. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\columnwidth]{figures/BDI_model_Human.pdf}
%     \caption{Jadex BDI execution model extended to raise or lower autonomy levels \ankit{replacing this will small simplified diagram.}}
%     \label{fig:bdi_human}
% \end{figure}

\ankit{add tables to show the mappings}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.98\columnwidth]{figures/REProcessANDMetaModelMapping.pdf}
%     \caption{First Attempt to create the RE process. Green nodes show the mapping to the meta-model. \ankit{Could you please provide a feedback on this - I can still =improve the "Autonomy Lower or Raise Autonomy Level" part.} \jch{Ankit -- This brute force model only gets us to the mappings, while I think we actually need the mappings and then a process for constructing the M1. Please see my comments in LaTeX. Creating this model is a great thought process though -- which should help us figure out the process we want to document in the paper.}}
%     % JCH Comments.
%     % This is basically a blunt force approach to map everything, and I don't think its very usable. To me, this is the raw information that *we* need (not the paper) to figure out a process.  I'd prefer a much simpler mapping of PQs to entities and then *well defined* steps i.e., a process for using those mappings to create an M1 from our metamodel.  So what could that process look like?
%     % We could easily forego the big diagram with some simple mappings under the PQs.  But the real question is how do we build the models from this?
%     %Can we identify which entities are involved and extract a skeleton M1 and then add meaningful labels.  Does that get us where we want to go?
    
%     \label{fig:my_label}
% \end{figure*}



